Proactive DP: A Multple Target Optimization Framework for DP-SGD

We introduce a multiple target optimization framework for DP-SGD referred to as pro-active DP. In contrast to traditional DP accountants, which are used to track the expenditure of privacy budgets, the pro-active DP scheme allows one to a-priori select parameters of DP-SGD based on a fixed privacy budget (in terms of $\epsilon$ and $\delta$) in such a way to optimize the anticipated utility (test accuracy) the most. To achieve this objective, we first propose significant improvements to the moment account method, presenting a closed-form $(\epsilon,\delta)$-DP guarantee that connects all parameters in the DP-SGD setup. We show that DP-SGD is $(\epsilon<0.5,\delta=1/N)$-DP if $\sigma=\sqrt{2(\epsilon +\ln(1/\delta))/\epsilon}$ with $T$ at least $\approx 2k^2/\epsilon$ and $(2/e)^2k^2-1/2\geq \ln(N)$, where $T$ is the total number of rounds, and $K=kN$ is the total number of gradient computations where $k$ measures $K$ in number of epochs of size $N$ of the local data set. We prove that our expression is close to tight in that if $T$ is more than a constant factor $\approx 4$ smaller than the lower bound $\approx 2k^2/\epsilon$, then the $(\epsilon,\delta)$-DP guarantee is violated. The above DP guarantee can be enhanced in thatDP-SGD is $(\epsilon, \delta)$-DP if $\sigma = \sqrt{2(\epsilon+\ln(1/\delta))/\epsilon}$ with $T$ at least $\approx 2k^2/\epsilon$ together with two additional, less intuitive, conditions that allow larger $\epsilon\geq 0.5$. Our DP theory allows us to create a utility graph and DP calculator. These tools link privacy and utility objectives and search for optimal experiment setups, efficiently taking into account both accuracy and privacy objectives, as well as implementation goals. We furnish a comprehensive implementation flow of our proactive DP, with rigorous experiments to showcase the proof-of-concept.

==> Section/01_Background_SGD_Hogwild_FLearning.tex <==
\section{Analysis general recursion}
%\label{app-rec}

%[TO DO: split up (1) SGD, Hogwild!, and general recursion with original definition tau, and (2) analysis strong convex]

The optimization problem for training many Machine Learning (ML) models using a training set $\{\xi_i\}_{i=1}^m$ of $m$ samples can be formulated as a finite-sum minimization problem as follows
\begin{equation}\label{eq:finite_sum_main}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \frac{1}{m}
\sum_{i=1}^m f(w; \xi_i) \right\}.
\end{equation}
The objective is to minimize a loss function with respect to model parameters $w$. This problem is known as empirical risk minimization and it covers a wide range of convex and non-convex problems from the ML domain, including, but not limited to, logistic regression, multi-kernel learning, conditional random fields and neural networks.
We are interested in solving the following more general stochastic optimization problem with respect to some distribution $\mathcal{D}$:
\begin{align}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \mathbb{E}_{\xi \sim \mathcal{D}} [ f(w;\xi) ] \right\},  \label{main_prob_expected_risk}  
\end{align}
where $F$ has a Lipschitz continuous gradient and $f$ has a \emph{finite lower bound} for every $\xi$.


The general form \eqref{main_prob_expected_risk} can be solved by using SGD as described in Algorithm \ref{sgd_algorithm}.
%~\citep{nguyen2018sgd}. 
 Thanks to its simplicity in implementation and efficiency in dealing with large scale datasets, stochastic gradient descent, originally introduced in \citep{RM1951}, has become the method of choice for solving not only (\ref{eq:finite_sum_main}) when $m$ is large but also (\ref{main_prob_expected_risk}).

\begin{algorithm}[ht]
  \caption{Stochastic Gradient Descent (SGD) Method}
  \label{sgd_algorithm}
\begin{algorithmic}[1]
  \State {\bfseries Initialize:} $w_0$
  \State {\bfseries Iterate:}
  \For{$t=0,1,2,\dots$}
  \State Choose a step size (i.e., learning rate) $\eta_t>0$. 
  \State Generate a random variable $\xi_t$.
  \State Compute a stochastic gradient $\nabla f(w_{t};\xi_{t}).$
  \State Update the new iterate $w_{t+1} = w_{t} - \eta_t \nabla f(w_{t};\xi_{t})$.
  \EndFor
\end{algorithmic}
\end{algorithm}


\subsection{The Hogwild! algorithm}
\label{app-rec}

To speed up SGD, an asynchronous SGD known as Hogwild! was introduced in~\citep{Hogwild}. 
Here, multiple computing threads work together and update shared memory in asynchronous fashion. The shared memory stores the most recently computed weight as a result of the SGD iterations computed by each of the computing threads.  Writes to and reads from vector positions in shared memory can be inconsistent. As a result a computing thread may start reading positions of the current weight vector from shared memory while these positions are updated by other computing threads out-of-order. Only writes to and reads from shared memory positions are considered atomic. This means that, when a computing thread reads the `current' weight vector from shared memory,  this weight vector is a mix of partial updates to the weight vector from other computing threads that executed previous SGD iterations. 
 
\citep{nguyen2018sgd,nguyen2018new}
%\citep{nguyen2018sgd,van2019characterization} 
introduce a general recursion for $w_t$.
% to which our analysis applies, next we will explain how the different variables in the recursion interact and describe two special cases, and finally we present pseudo code of the algorithm using the recursion.  
The recursion explains which positions in $w_t$ should be updated in order to compute $w_{t+1}$. Since $w_t$ is stored in shared memory and is being updated in a possibly non-consistent way by multiple cores who each perform recursions, the shared memory will contain a vector $w$ whose entries represent a mix of updates. That is, before performing the computation of a recursion, a computing thread will first read  $w$ from shared memory, however, while reading $w$ from shared memory, the entries in $w$ are being updated out of order. The final vector $\hat{w}_t$ read by the computing thread represents an aggregate of a mix of updates in previous iterations.

The general recursion (parts of text extracted from \citep{nguyen2018new}) is defined as follows: For $t\geq 0$,
\begin{equation}
 w_{t+1} = w_t - \eta_t d_{\xi_t}  S^{\xi_t}_{u_t} \nabla f(\hat{w}_t;\xi_t),\label{eqwM}
 \end{equation}
 where
 \begin{itemize}
 \item $\hat{w}_t$ represents the vector used in computing the gradient $\nabla f(\hat{w}_t;\xi_t)$ and whose entries have been read (one by one)  from  an aggregate of a mix of  previous updates that led to $w_{j}$, $j\leq t$, and
 \item the $S^{\xi_t}_{u_t}$ are diagonal 0/1-matrices with the property that there exist real numbers $d_\xi$ satisfying
\begin{equation} d_\xi \mathbb{E}[S^\xi_u | \xi] = D_\xi, \label{eq:SexpM} \end{equation}
where the expectation is taken over $u$ and $D_\xi$ is the diagonal 0/1 matrix whose $1$-entries correspond to the non-zero positions in $\nabla f(w;\xi)$ in the following sense: The $i$-th entry of $D_\xi$'s diagonal is equal to 1 if and only if there exists a $w$ such that the $i$-th position of $\nabla f(w;\xi)$ is non-zero. 
\end{itemize}

The role of matrix $S^{\xi_t}_{u_t}$ is that it filters which positions of gradient $\nabla f(\hat{w}_t;\xi_t)$ play a role in (\ref{eqwM}) and need to be computed. Notice that $D_\xi$ represents the support of $\nabla f(w;\xi)$; by $|D_\xi|$ we denote the number of 1s in $D_\xi$, i.e., $|D_\xi|$ equals the size of the support of $\nabla f(w;\xi)$.

We restrict ourselves to choosing (i.e., fixing a-priori) {\em non-empty} matrices  $S^\xi_u$ that ``partition'' $D_\xi$ in $D$ approximately ``equally sized'' $S^\xi_u$: 
$$ \sum_u S^\xi_u = D_\xi, $$
where each matrix $S^\xi_u$ has either $\lfloor |D_\xi|/D \rfloor$ or $\lceil |D_\xi|/D \rceil$ ones on its diagonal. We uniformly choose one of the matrices $S^{\xi_t}_{u_t}$ in (\ref{eqwM}), hence, $d_\xi$ equals the number of matrices $S^\xi_u$, see (\ref{eq:SexpM}).

In order to explain recursion (\ref{eqwM}) we  consider two special cases. For $D=\bar{\Delta}$, where 
$$ \bar{\Delta} = \max_\xi \{ |D_\xi|\}$$
represents the maximum number of non-zero positions in any gradient computation $f(w;\xi)$, we have that for all $\xi$, there are exactly $|D_\xi|$ diagonal matrices $S^\xi_u$ with a single 1 representing each of the elements in $D_\xi$. Since  $p_\xi(u)= 1/|D_\xi|$ is the uniform distribution, we have $\mathbb{E}[S^\xi_u | \xi] = D_\xi / |D_\xi|$, hence, $d_\xi = |D_\xi|$. This gives the recursion
\begin{equation}
 w_{t+1} = w_t - \eta_t |D_\xi|  [ \nabla f(\hat{w}_t;\xi_t)]_{u_t},\label{eqwM1}
 \end{equation}
 where $ [ \nabla f(\hat{w}_t;\xi_t)]_{u_t}$ denotes the $u_t$-th position of $\nabla f(\hat{w}_t;\xi_t)$ and where $u_t$ is a uniformly selected position that corresponds to a non-zero entry in  $\nabla f(\hat{w}_t;\xi_t)$.
 
At the other extreme, for $D=1$, we have exactly one matrix $S^\xi_1=D_\xi$ for each $\xi$, and we have $d_\xi=1$. This gives the recursion
\begin{equation}
 w_{t+1} = w_t - \eta_t  \nabla f(\hat{w}_t;\xi_t).\label{eqwM2}
 \end{equation}
Recursion (\ref{eqwM2}) represents Hogwild!. In a single-thread setting where updates are done in a fully consistent way, i.e. $\hat{w}_t=w_t$, yields SGD. 


%. Experiments in Section \ref{sec_experiments} indicate that while the expected convergence rates do seem to look similar, their variances differ.
 
 Algorithm \ref{HogWildAlgorithm} gives the pseudo code corresponding to recursion (\ref{eqwM}) with our choice of sets $S^\xi_u$ (for parameter $D$).
 
 \begin{algorithm}
\caption{Hogwild! general recursion}
\label{HogWildAlgorithm}
\begin{algorithmic}[1]

   \State {\bf Input:} $w_{0} \in \mathbb{R}^d$
   \For{$t=0,1,2,\dotsc$ {\bf in parallel}} 
    
  \State read each position of shared memory $w$
  denoted by $\hat w_t$  {\bf (each position read is atomic)}
  \State draw a random sample $\xi_t$ and a random ``filter'' $S^{\xi_t}_{u_t}$
  \For{positions $h$ where $S^{\xi_t}_{u_t}$ has a 1 on its diagonal}
   \State compute $g_h$ as the gradient $\nabla f(\hat{w}_t;\xi_t)$ at position $h$
   \State add $\eta_t d_{\xi_t} g_h$ to the entry at position $h$ of $w$ in shared memory {\bf (each position update is atomic)}
   \EndFor
   \EndFor
\end{algorithmic}
\end{algorithm}



In order to use Algorithm \ref{HogWildAlgorithm} in federated learning, we use the following reinterpretation of shared memory and computing threads.
Clients in FL represent the different computing threads. The server plays the role of shared memory where locally  computed weight vectors at the clients are `aggregated' as in (\ref{eqwM}). Each Client$_j$  first receives each of the entries of the weight vector $w$ currently stored at the server. This is done by successive atomic reads from $w$ as described above. Next the collected entries form together a vector $\hat{w}_t$ and the gradient $\nabla f(\hat{w}_t;\xi_t)$ for some sample $\xi_t \sim {\mathcal D}$ is computed. The gradient multiplied by a step size $\eta_t$ and correction factor $d_{\xi_t}$ is subtracted from the weight vector stored at the server. This is done by a series of successive atomic writes. Each of the clients (just like the computing threads above) work in parallel continuously updating entries in the weight vector $w$ stored at the server. %In Section \ref{FLalg} we will explain how communication can be partitioned in rounds by grouping reads and writes together.

In the context of different computing threads atomically reading and writing entries of vector $w$ from shared memory, we define the amount of asynchronous behavior by parameter $\tau$ as in \citep{nguyen2018new}:
%\begin{ass}[Consistent with delay $\tau$]
%\label{ass_tau}

\begin{defn} 
We say that weight vector $w$ stored at the server is {\em consistent with delay $\tau$}  with respect to recursion (\ref{eqwM}) if, for all $t$, vector $\hat{w}_t$ includes the aggregate of the updates up to and including those made during the $(t-\tau)$-th iteration (where (\ref{eqwM}) defines the $(t+1)$-st iteration). Each position read from shared memory is atomic and each position update to shared memory is atomic (in that these cannot be interrupted by another update to the same position).
\end{defn}
%\end{ass}

Even though this (original) definition does not consider $\tau$ as a function of the iteration count $t$, the next subsections do summarize how $\tau$ can depend as a function on $t$.





==> Section/03_Unified_Framework_FL_Hogwild.tex <==
%% \usepackage{svg}
%\section{Convergence Rate for Strongly Convex Problems}


%\begin{ass}[$L$-smooth]
%\label{ass_smooth}
%$f(w;\xi)$ is $L$-smooth for every realization of $\xi$, i.e., there exists a constant $L > 0$ such that, $\forall w,w' \in \mathbb{R}^d$, 
%\begin{align*}
%\| \nabla f(w;\xi) - \nabla f(w';\xi) \| \leq L \| w - w' \|. \label{eq:Lsmooth_basic}
%\end{align*} 
%\end{ass}

%\begin{ass}\label{ass_convex}
%$f(w;\xi)$ is convex for every realization of $\xi$, i.e., $\forall w,w' \in \mathbb{R}^d$, 
%\begin{gather*}
%f(w;\xi)  - f(w';\xi) \geq \langle \nabla f(w';\xi),(w - w') \rangle.
%\end{gather*}
%\end{ass}

%\begin{ass}[$\mu$-strongly convex]
%\label{ass_stronglyconvex}
%The objective function $F: \mathbb{R}^d \to \mathbb{R}$ is a $\mu$-strongly convex, i.e., there exists a constant $\mu > 0$ such that $\forall w,w' \in \mathbb{R}^d$, 
%\begin{gather*}
%F(w) - F(w') \geq \langle \nabla F(w'), (w - w') \rangle + \frac{\mu}{2}\|w - w'\|^2. \label{eq:stronglyconvex_00}
%\end{gather*}
%\end{ass}

%\begin{ass}[Finite $\sigma$]
%\label{ass_finitesigma}
%Let $\sigma^2 =  \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$ where $w_{*} = \arg \min_w F(w)$. It is required that $\sigma^2 < \infty$. 
%\end{ass}

%\begin{ass}[Consistent with delay $\tau$]
%\label{ass_tau_consistent}
%We say that shared memory is consistent with delay $\tau$  with respect to recursion (\ref{eqwM}) if, for all $t$, vector $\hat{w}_t$ includes the aggregate of the updates up to and including those made during the $(t-\tau)$-th iteration (where (\ref{eqwM}) defines the $(t+1)$-st iteration). Each position read from shared memory is atomic and each position update to shared memory is atomic (in that these cannot be interrupted by another update to the same position).
%\end{ass}


%\vspace{3pt}
%\noindent
%{\bf Constant Step Sizes:}
%we borrow the theoretical result on analysis of Hogwild! with constant step size scheme $\eta_t= \eta, \forall t$ from~\citep{leblond2018improved}.

%\begin{ass}[Upper bound on $\tau$ - page 26~\citep{leblond2018improved} ]
%\label{ass_tau}
%For given Hogwild! algorithm with constant step size $\eta$ and $F$ $\mu$-strongly convex, it requires:
%\begin{equation}
%\label{tau2}   
%\tau \leq \frac{1}{\mu \eta}.
%\end{equation}
%\end{ass}



%In~\citep{leblond2018improved}, $F$ is a finite sum problem, i.e., 
%by defining  $f_i(w) := f(w;\xi_{i})$,   
%\begin{gather}\label{main_prob}
%\min_{w \in \mathbb{R}^d} \left\{ F(w) = \frac{1}{m} \sum_{i=1}^m f_i(w) \right\}.  
%\end{gather}

%Moreover, $F$ is $\mu$-strongly convex (Assumption~\ref{ass_stronglyconvex}), component function $f_i(w)$ is convex and $L$-smooth (i.e., Assumptions~\ref{ass_convex} and~\ref{ass_smooth}), and $\sigma^2 < \infty$ (Assumption~\ref{ass_finitesigma}) and $\tau \leq \frac{1}{\mu \eta}$ (Assumption~\ref{ass_tau}) with Assumption~\ref{ass_tau_consistent}. Let us denote $\Delta$ as sparsity parameter as in Definition 7 in~\citep{leblond2018improved} and $\Delta\in [\frac{1}{m},1]$. As explained in~\citep{leblond2018improved}, this parameter depends on the Hogwild! system, i.e., the application and the definition of atomic write.    

%Let $a(\tau)=\frac{1}{5(1+2\tau \sqrt{\Delta})\zeta(\kappa,\Delta,\tau)}$ where $\zeta(\kappa,\Delta,\tau)=\sqrt{1+\frac{1}{2\kappa}\min\{\frac{1}{\sqrt{\Delta}},\tau\}}$ and $\kappa=\frac{L}{\mu}$. For any step size $\eta=\frac{a}{L}$ with $a\leq \min\{a(\tau),\frac{\kappa}{\tau}\}$ and $\rho=\frac{a}{\kappa}$, we have:
% \begin{equation}
%     \mathbb{E}[\|\hat{w}_t - w_*\|^2]\leq (1-\rho)^t(2\|w_0-w_*\|^2) + b,
% \end{equation}
% where 
% \begin{eqnarray*}
% b&=&(\frac{8\eta(C_1+\tau C_2)}{\mu} + 4\eta^2C_1\tau )\sigma^2,\\
% C_1 &=& 1 + \sqrt{\Delta}\tau, \\
% C_2 &=& \sqrt{\Delta} + \eta \mu C_1.
% \end{eqnarray*}
%% \end{thm}
%% 


%\vspace{3pt}
%\noindent
%{\bf Diminishing Step Sizes}
%In~\citep{nguyen2018sgd}, the authors study the convergence of Hogwild! with Assumptions~\ref{ass_smooth},~\ref{ass_stronglyconvex},~\ref{ass_finitesigma}, and ~\ref{ass_tau_consistent} for diminishing step size schemes which can allows us to find the true optimal solution $w_*$. 


%Algorithm~\ref{HogWildAlgorithm} for diminishing step sizes $\eta_t = \frac{\alpha_t}{\mu(t+E)}$ with $4\leq \alpha_t \leq\alpha$ and $E = \max\{ 2\tau, \frac{4 L \alpha D}{\mu}\}$ has the following properties, see \citep{nguyen2018sgd,nguyen2018new}: The expected number of single vector entry updates after $t$ iterations is equal to $t' = t \bar{\Delta}_D /D$ with  $\bar{\Delta}_D = D \cdot \mathbb{E}[\lceil |D_\xi|/D \rceil]$ and both convergence rates $ \mathbb{E}[\|\hat{w}_{t} - w_* \|^2]$ and $\mathbb{E}[\|w_{t} - w_* \|^2]$ are at most
%$$\frac{4\alpha^2D N}{\mu^2} \frac{t}{(t + E - 1)^2} + O\left(\frac{\ln t}{(t+E-1)^{2}}\right).$$
% In terms of the expected number $t'$ of  single vector entry updates after $t$ iterations, both $\mathbb{E}[\|\hat{w}_{t} - w_* \|^2]$ and $\mathbb{E}[\|w_{t} - w_* \|^2]$ are at most
%$$\frac{4\alpha^2 \bar{\Delta}_D N}{\mu^2} \frac{1}{t'} + O\left(\frac{\ln t'}{t'^{2}}\right).$$


%The leading term of the upper bound on the convergence rate is independent of delay $\tau$. 

%In fact we may allow $\tau$ to be a monotonic increasing function of $t$ with
%\begin{equation}
%\frac{2 L \alpha D}{\mu}\leq \tau(t)\leq \sqrt{\frac{t}{\ln t}  \cdot \left( 1 - \frac{1}{\ln t} \right)} \label{tau1}
%\end{equation}
%(this will make $E = \max\{ 2\tau(t), \frac{4 L \alpha D}{\mu}\}$ also a function of $t$). In terms of asymptotics in $t$, if  $12\leq \alpha_t\leq \alpha$, then the leading term of the convergence rate for such $\tau$ as a function of $t$ does not change while the second order terms increase to $O(\frac{1}{t\ln t})$. It turns out that if $\tau(t)$ is set to meet the upper bound in (\ref{tau1}), then for large enough $t\geq T_0 =  \exp[ 2\sqrt{\Delta}(1+\frac{(L+\mu)\alpha}{\mu})]$
%the constants of all the asymptotic higher order terms that contain $\tau(t)$ are such that the concrete values of all these terms are at most the leading term of the convergence rate.\footnote{For completeness, the leading term is also independent of $\|w_0-w_*\|^2$ -- it turns out that for $t \geq T_1 = \frac{\mu^2}{\alpha^2 N D}\|w_0-w_*\|^2$ the higher order term that contains $\|w_0-w_*\|^2$ is at most the leading term.}
% So, for the worst-case delay function $\tau(t)$ we have for $t\geq T_0$ that the convergence rate is at most a constant times $\frac{4\alpha^2D N}{\mu^2} \frac{t}{(t + E - 1)^2}$. In practice, we expect to see this behavior for much smaller $T_0$. Also, if $\tau(t)$ is a much less increasing function in $t$, we expect to be able to prove a much smaller $T_0$.


%The upper bounds on the convergence rates above are tight as shown in \citep{nguyen2019tight}.

%\vspace{3pt}
%\noindent
%{\bf Delay $\tau$:}
%%For diminishing stepsizes, $\tau$ may increase as much as indicated by (\ref{tau1}) without affecting the optimality of the convergence rate. Similarly, for fixed stepsizes, $\tau$ can be at most a constant upper bound (\ref{tau2}) without affecting the optimality of the convergence rate. We propose to use this flexibility in $\tau$ to map the Hogwild! algorithm to federated learning where server/clients rounds can be asynchronous (and yet we are still able to adapt above convergence rate results).

%\section{Our Method}


%The optimization problem for training many Machine Learning (ML) models using a training set $\{\xi_i\}_{i=1}^m$ of $m$ samples can be formulated as a finite-sum minimization problem as follows
%$$ 
%\min_{w \in \mathbb{R}^d} \left\{ F(w) = \frac{1}{m}
%\sum_{i=1}^m f(w; \xi_i) \right\}.
%$$
%The objective is to minimize a loss function with respect to model parameters $w$. This problem is known as empirical risk minimization and it covers a wide range of convex and non-convex problems from the ML domain, including, but not limited to, logistic regression, multi-kernel learning, conditional random fields and neural networks.
%We are interested in solving the following more general stochastic optimization problem with respect to some distribution $\mathcal{D}$:
%\begin{align}
%\min_{w \in \mathbb{R}^d} \left\{ F(w) = \mathbb{E}_{\xi \sim \mathcal{D}} [ f(w;\xi) ] \right\},  \label{eqObj}  
%\end{align}
%where $F$ has a Lipschitz continuous gradient and $f$ is bounded from below for every $\xi$.


%Our approach is based on the Hogwild!~\citep{nguyen2018sgd} recursion 
%\begin{equation}
% w_{t+1} = w_t - \eta_t  \nabla f(\hat{w}_t;\xi_t),\label{eqwM2a}
% \end{equation}
% where $\hat{w}_t$ represents the vector used in computing the gradient $\nabla f(\hat{w}_t;\xi_t)$ and whose vector entries have been read (one by one)  from  an aggregate of a mix of  previous updates that led to $w_{j}$, $j\leq t$.
% In a single-thread setting where updates are done in a fully consistent way, i.e. $\hat{w}_t=w_t$, yields SGD with diminishing step sizes $\{\eta_t\}$. 
%Recursion (\ref{eqwM2a}) models asynchronous SGD. We define the amount of asynchronous behavior by a function $\tau(t)$:


%\begin{defn}
%We say that the sequence $\{w_t\}$  is {\em consistent with delay function $\tau$}  %with respect to recursion (\ref{eqwM2}) 
%if, for all $t$, vector $\hat{w}_t$ includes the aggregate 
%of the updates up to and including those made during the $(t-\tau(t))$-th iteration\footnote{ (\ref{eqwM2a}) defines the $(t+1)$-th iteration, where $\eta_t\nabla f(\hat{w}_t;\xi_t)$ represents the $(t+1)$-th update.}, i.e., $\hat{w}_t = w_0 - \sum_{j\in {\cal U}} \eta_j \nabla f(\hat{w}_j;\xi_j)$ for some ${\cal U}$ with $\{0,1,\ldots, t-\tau(t)-1\}\subseteq {\cal U}$.
%\end{defn}

%TO DO: talk about delay quickly, mention in this context the rebuttal of AISTATS showing that large sample sizes are of interest and also increasing sample size sequences -- which our theory covers (no experiments)

%TO DO: Only procedure MainClient -- Let's call it local SGD. 12-14 replaced by text -- invariant om delay may require some waiting. Explain that the adaptations are from DP paper -- our theory generalizes theirs and hence also applies to their algorithm, it is all pretty much the same.

%TO DO Remove subscript $c$ everywhere in analysis etc.

%It turns out that for strong convex problems an optimal convergence rate for diminishing step sizes can be achieved for $\tau(t)$ as large as $\approx \sqrt{t/\ln t}$ (for a precise formulation see
%Supplemental Material \ref{app-sc-dim}).
%In order words, the recursion can resist large amounts of asynchronous behavior. In practice such amounts of asynchronous behavior will not occur. Our key idea is to  design {\em a distributed SGD algorithm which introduces additional asynchronous behavior} (because we can resist it anyway) by having the algorithm communicate less with the central server. This has as main advantage less communication and when combined with Differential Privacy (DP) less aggregated added DP noise is needed (leading to faster convergence to a model with desired accuracy). For the same DP guarantees and the same number of iterations (grad computations) we obtain better accuracy and have less communication.

%\subsection{Differential Private Asynchronous distributed SGD}
% \subsection{Asynchronous solution}





%Clients update their local models according to
%Algorithm \ref{alg:DP}, where we discard lines 17, 23, and 24 indicated by NEW; these additions are analysed in  the next section.
%Supplemental Material \ref{app-alg} has all the detailed pseudo code with annotated invariants.

%TO DO: move start to appendix, initializing $s_{i,c}$ to appendix, in algorithm add ISRReceive (Server broadcasts a new global model $\hat{v}_k$ once the updates for a next sample round from all clients has been received and aggregated), add Setup in words, add notation c,i,h to w.

%We propose to have a server to maintain a global model which is updated according to Algorithm \ref{alg:server}. The server receives updates from clients who work on local models by executing Algorithm \ref{alg:client}. Before any computation starts both server and clients agree on the used diminishing step size sequence, the increasing sample (mini batch) sequences, initial default global model, and permissible delay function $\tau$, see Algorithm \ref{alg:setup}.

%The clients in the distributed computation  apply recursion (\ref{eqwM2a}) in lines 16, 19, 20. We want to label each recursion with an iteration count $t$; this can then be used to compute with which delay function the labeled sequence $\{w_t \}$ is consistent.
%In  order to find an ordering based on $t$ we define in Supplemental Material \ref{appmain} a mapping $\rho$ from the annotated labels $(c,i,h)$ in \Call{MainClient}{} to $t$ and use this to prove:

%Idea is to find an ordering of recursions that maps to this recursion and compute the corresponding delay
%
%[TO DO: put the next part in appendix and relate $w_{i,c,h}$ to $w_t$, and state theorem]
%$$\rho(c,i,h)= (\sum_{l < i} s_{l}) + \min\{ t' \ : \ h=|\{ t\leq t' \ : \ a(i,t)=c\}|\} ,$$ 
%where sequence sample size sequence $\{s_i\}$ and labelling function $a(.,.)$ are defined in \Call{Setup}{}.

%Notice that given $t$, we can compute $i$ as the largest index for which $\sum_{l<i} s_{l} \leq t$, compute $t'=t- \sum_{l<i} s_{l}$ and $c=a(i,t')$, and compute $h=|\{ t\leq t' \ : \ a(i,t)=c\}|$. This procedure inverts $\rho$ since $\rho(c,i,h)=t$, hence, $\rho$ is bijective.  We use $\rho$ to order local models $\hat{w}_{c,i,h}$ by writing $\hat{w}_t=\hat{w}_{c,i,h}$ with $t=\rho(c,i,h)$. Similarly, we write $\xi_t= \xi_{c,i,h}$ for local training data samples. 

%Give a mapping

%Explain algorithm annotation and invariants
%From the invariant in \Call{MainServer}{} we infer that  $\hat{v}_k$ includes all the aggregate updates $U_{i,c}$ for $i< k$ and $c\in {1,\ldots n}$. See Algorithm \ref{alg:client} for the clients, 
%$$\sum_{c\in \{1,\ldots, n\}} U_{i,c} = \sum_{c\in \{1, \ldots, n\}} \sum_{h=0}^{s_{i,c}-1} g_{c,i,h} \mbox{ with } g_{c,i,h}= \nabla f(\hat{w}_{c,i,h}; \xi_{c,i,h}).$$
%By using mapping $\rho$, this is equal to
%\begin{eqnarray*}
%\sum_{c\in \{1, \ldots, n\}} \sum_{h=0}^{s_{i,c}-1} \nabla f(\hat{w}_{c,i,h}; \xi_{c,i,h}) &=&
%\sum_{c\in \{1, \ldots, n\}} \sum_{h=0}^{s_{i,c}-1} \nabla f(\hat{w}_{\rho(c,i,h)}; \xi_{\rho(c,i,h)}) \\
%&=& \sum_{t=s_0+\ldots s_{i-1}}^{s_0+\ldots+s_i-1} \nabla f(\hat{w}_{t}; \xi_{t}).
%\end{eqnarray*}
%This implies that 
%%$\sum_{(i,c,j)\in H} \eta_i U_{i,c}$, and therefore also 
%$\hat{v}_k$, includes all the gradient updates (across all clients) that correspond to $\hat{w}_t$ for $t\leq s_0+\ldots+s_{k-1}-1= t_{glob}-t_{delay}$ in the notation of \Call{MainClient}{}.
%%}

%Let $\rho(c,i,h)=t$. Notice that $t= \rho(c,i,h) \leq s_0+ \ldots + s_i -(s_{i,c}-h)-1=t_{glob}$. In \Call{MainClient}{} we wait as long as $\tau(t_{glob})= t_{delay}$. This means that $h$ will not further increase until $k$ increases in client $c$'s \Call{ISRReceive}{} when a new global model is received. This implies $t_{delay}\leq \tau(t_{glob})$ as an invariant of the algorithm. Because $t-\tau(t)$ is an increasing function in $t$, the derived inequality implies  $t-\tau(t)\leq t_{glob}-\tau(t_{glob}) \leq t_{glob}-t_{delay}$. Notice that $\hat{w}_t=\hat{w}_{c,i,h}$  includes the updates aggregated in $\hat{v}_k$ as last received by client $c$'s \Call{ISRReceive}{}. We concluded above that $\hat{v}_k$ includes all gradient updates that correspond to gradient computations up to iteration count $t_{glob}-t_{delay}$. This includes gradient computations up to iteration count $t-\tau(t)$. Therefore, the computed sequence $\{w_t\}$ is consistent with delay function $\tau$.

%As a second consequence of mapping $\rho$ we notice that $\{\xi_t\}=\{\xi_{c,i,h}\}$. In fact $\xi_t=\xi_{c,i,h}$ for $(c,i,h)=\rho^{-1}(t)$. %This relation is based on mapping $a(i,t)=c$ as
%Notice that \Call{Setup}{} constructs the mapping $a(i,t)=c$  which is used to define $\rho$. Mapping $a(i,t)$ represents a random table of client assignments $c$ generated by using a probability vector $(p_1,\ldots, p_n)$ (with $c$ being selected with probability $p_c$ for the $(i,t)$-th entry). So, $\xi_t\sim {\cal D}_c$ in \Call{MainClient}{} with probability $p_c$. This means that $\xi_t\sim {\cal D}$ with ${\cal D} = \sum_{c=1}^n p_c {\cal D}_c$.

%%each is equal to a ... random choice according to $p_c$ .. ${\cal D}$ .. objective function.

%\begin{thm} \label{thmalg}
%Our setup, client, and server algorithms produce a sequence $\{w_t\}$ according to recursion (\ref{eqwM2a}) where $\{\xi_t\}$ are selected from distribution ${\cal D}=\sum_{c=1}^n p_c {\cal D}_c$. Sequence $\{w_t\}$ is consistent with delay function $\tau$ as defined in \Call{Setup}{}.
%and where $\xi_t\sim {\cal D}$
%\end{thm}

%From the invariant in \Call{MainServer}{} we infer that $\hat{w}_t$ includes the aggregate of updates $\sum_{i=1}^k\sum_{c=1}^n \eta_i U_{i,c}$

%TO DO numbering i from 0.

%This shows that the delay for gradient computations is at most $t_i$ (since the last received global model includes the first $s_0+\ldots +s_k$ gradient computations.



%lemma: delay




==> Section/04_Convergence_Analysis.tex <==
\section{Convergence Analysis}

\subsection{Convergence Analysis of Hogwild!}
% We will focus on an important special case of the problem, characterized by $F$ being a strongly convex function over some convex domain $\mathbb{W}$ (which is assumed to be a subset of some Hilbert space) \cite{rakhlin2011making}.

% A function $F$ is $\mathbb{L}$-smooth if it is differentiable and has Lipschitz gradients,
% \begin{align}
% \nabla F(w\;') - \nabla F(w) \leq \mathbb{L}\norm{w\;' - w}
% \end{align}
% where $\mathbb{L} > 0$ and $\forall w, w\;' \in \mathbb{R}^d$

% % http://www.rpi.edu/dept/arc/training/latex/LaTeX_symbols.pdf
% Formally, we also say that a function $F$ is $\lambda$-strongly convex, if for all $w$, $w\;'\in \mathbb{W}$ and any subgradient $g$ of $F$ at $w$,
% \begin{align}
% F(w\;') \geq F(w) + \langle g, w\;' - w \rangle  + \frac{\lambda}{2}\norm{w\;' - w}^2
% \end{align}

% We define the (unique) optimal solution of $F$ as $w^{*}$. Formally, a function $F$ is $\mu$-smooth with respect to $w^{*}$ if for all $w \in \mathbb{W}$,
% \begin{align}
% F(w) - F(w^{*}) \leq \frac{\mu}{2}\norm{w - w^{*}}^2
% \end{align}

% Such functions arise, for instance, in logistic and least squares regression, and in general for learning linear predictors where the loss function has a Lipschitz continuous gradient.

% The paper in \cite{leblond2018improved} states the theoretical results of their analysis of Hogwild! with inconsistent reads and writes in the framework.

% \theoremstyle{definition}
% \begin{definition}\label{SGDbounded}
% Let $\sigma^2$ = $\mathbb{E}$ $\norm{f_{i}\;' (w^{*})}^2$ be the variance of the gradient estimator at the optimum. The classical theoretical analysis of SGD assumes that the stochastic gradients are uniformly bounded, i.e. there exists a finite (fixed) constant $\sigma < \infty$, such that:
% $\mathbb{E} \norm{\nabla F(w)}^2 \leq \sigma^2$ \cite{nguyen2018sgd}.

% \end{definition}

% For reference, we start by giving the rate of convergence of serial SGD \cite{schmidt2014convergence}.

% \theoremstyle{definition}
% \begin{definition}
% As in \cite{recht}, we introduce $\triangle_{r} := \max_{v \in (1..d)}$ $|$ ${i:v \in S_{i}} |$. $\triangle_{r}$ is the maximum right-degree in the bipartite graph of the factors and the dimensions, i.e., the maximum number of data points with a specific feature. For succinctness, we also define $\triangle := \frac{\triangle_{r}}{n}$. We have $1 \leq \triangle{r} \leq n$, and hence $\frac{1}{n} \leq \triangle \leq 1$.
% \end{definition}

% \begin{assumption}{\textbf{(bounded overlaps)}}
% We assume that there exists a uniform bound, called $\tau$, on the maximum number of iterations that can overlap together. We say that iterations $r$ and $t$ overlap if at some points they are processed concurrently. One iteration is being processed from the start of the reading of the shared parameters to the end of the writing of its update. The bound $ \tau$ means that iterations $r$ cannot overlap with iteration $t$ for $r \geq t + \tau + 1$, and thus that every coordinate update from iteration $t$ is successfully written to memory before the iteration $t + \tau + 1$ starts.
% \end{assumption}

% \theoremstyle{definition}
% \begin{theorem}{\textbf{Convergence guarantee and rate of SGD}}
% Let a $\leq$ $\frac{1}{2}$. Then  for any step size $\gamma = \frac{a}{\mathbb{L}}$, SGD converges in expectation to $b$-accuracy at a geometric rate of at least: $\rho(a) = \frac{a}{\kappa}$, i.e, $\mathbb{E}$ $\norm{x_{t} - x^{*}}^2 \leq (1 - \rho)^{t} \norm{x_{t} - x^{*}}^2$ + $b$ with $b = 2\frac{\gamma \sigma^2}{\mu}$ and satisfies $\mu$-strong requirement.
% \end{theorem}

% As SGD only converges linearly up to a ball around the optimum, to make sure we reach $\epsilon$-accuracy, it is necessary that $2\frac{\gamma \sigma^2}{\mu} \leq \epsilon$, i.e, $\gamma \leq \frac{\epsilon \mu}{2 \sigma^2}$. All told, in order to get linear convergence to $\epsilon$-accuracy, serial SGD requires $\gamma \leq \min\{\frac{1}{2 \mathbb{L}},\frac{\epsilon \mu}{2 \sigma^2}\}$

% We define the update $gt_t := g(\hat{x}_t,\hat{\alpha}_t,i_t)$, is an unbiased estimator of the true gradient at $\hat{x}_t$ in conditional expectation. For all $t > 0$,

% $a_{t+1} \leq (1 - \frac{\gamma \mu}{2}) a_t + \gamma^2 C_1 \mathbb{E} \norm{g_t}^2 + \gamma^2 C_2 \sum_{u=t-\tau}^{t-1} \mathbb{E}\norm{g_u}^2 + 2\gamma e_t$,
% where $C_1 := 1 + \sqrt{\triangle_{r}}$ and $C_2 := \sqrt{\triangle} + \gamma \mu C_1$.

% \theoremstyle{definition}
% \begin{theorem}{\textbf{Convergence guarantee and rate of Hogwild!}}\label{Hogwild}
% Let $a^{*}(\tau) := $ $\frac{1}{5(1 + 2\tau\sqrt{\triangle}) \xi(\kappa, \triangle, \mathbb{T})}$ where $\xi(\kappa, \triangle, \mathbb{T}) := \sqrt{1 + \frac{1}{2 \kappa} \min(\frac{1}{\sqrt{\triangle}}}, \tau)$, note that $\xi(\kappa, \triangle, \mathbb{T}) \approx 1$ unless $\kappa < \frac{1}{\sqrt{\triangle}} (\leq \sqrt{n})$.

% For any step size $\gamma = \frac{a}{\mathbb{L}}$ with $a < \min\{a^{*}(\tau), \frac{\kappa}{\tau}\}$, the inconsistent read iterates of $Algorithm$ 1 converge in expectation to $b$-accuracy at a geometric rate of at least: $\rho(a) = \frac{a}{\kappa}$, i.e, $\mathbb{E}$ $\norm{x_{t} - x^{*}}^2 \leq (1 - \rho)^{t} (2\norm{x_{0} - x^{*}}^2$) + $b$, where we define $b = \epsilon^{2}(\frac{8\gamma(C_{1} + \tau C_{2})}{\mu} + 4 \gamma^{2} C_{1}\tau)$ and and $C_1$ and $C_2(\gamma)$ are defined above.
% \end{theorem}

% Once again this result is quite close to the one obtained for serial SGD. Note that we recover this exact condition (up to a small constant factor) if we set $\tau = 0$, i.e. if we force our asynchronous algorithm to be serial.

% \begin{corollary}[\textbf{Speedup condition}]
% Suppose $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\kappa\})$. Then for any step size $\gamma \leq \frac{a^{*}(\tau)}{\mathbb{L}} = \mathcal{O}(\frac{1}{\mathbb{L}})$ (i.e., any allowable step size for SGD), Hogwild! converges geometrically to a ball of radius $r_h = \mathcal{O}(\frac{\gamma \sigma^2}{\mu})$ with rate factor $\rho = \frac{\gamma \mu}{2}$ (similar to SGD), and is thus linearly faster than its sequential counterpart up to a constant factor.

% Moreover, a universal step size of $\Theta(\frac{1}{\mathbb{L}})$ can be used for Hogwild! to be adaptive to local strong convexity with a similar rate to SGD (i.e., knowledge of $\kappa$ is not required).
% \end{corollary}

% If $\gamma = \mathcal{O}(\frac{1}{\mathbb{L}})$, Hogwild! obtains the same convergence rate as SGD and converges to a ball of equivalent radius. Since the maximum step size guaranteeing linear convergence for SGD is also $\mathcal{O}(\frac{1}{\mathbb{L}})$, Hogwild! is linearly faster than SGD for any reasonable step size – under the condition that $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\kappa\})$. We also remark that since $\gamma \leq \frac{1}{\mathbb{L}}$ and $\tau \leq \kappa$, we have $\gamma \mu \tau \leq 1$, which means the condition $a \leq \frac{\kappa}{\mu}$ is superseded by $a \leq a^{*}(\tau)$ in $\ref{Hogwild}$.

% The papers in \cite{leblond2018improved,mania2017perturbed} noted that our results are derived directly on iterates, that is, we bound the distance between $x_t$ and $x^{∗}$. We can easily obtain results on function values to bound $\mathbb{E}[f(x_t) - f(x^*)]$ by adapting the classical smoothness inequality: $\mathbb{E}[f(x_t) - f(x^*)] \leq \mathbb{E}\norm{x_t - x^*}^2$ to the asynchronous parallel setting.

% \textbf{Convergence to $\epsilon$-accuracy.}
% As noted in \cite{mania2017perturbed}, for our algorithm to converge to $\epsilon$-accuracy for some $\epsilon > 0$, we require an additional bound on the step size to make sure that the radius of the ball to which we converge is small enough. For SGD, this means using a step size $\gamma = \mathcal{O}(\frac{\epsilon \mu}{\sigma^2})$. We can also prove that under the conditions that $\tau = \mathcal{O}(\frac{1}{\sqrt{\triangle}})$ and $\gamma \mu \tau \leq 1$, Hogwild! requires the same bound on the step size to converge to $\epsilon$-accuracy. If $\epsilon$ is small enough, the active upper bound on the step size is $\gamma = \mathcal{O}(\frac{\epsilon \mu}{\sigma^2})$ for both algorithms. In this regime, we obtain a relaxed condition on τ for a linear speedup. The condition $\tau \leq \kappa$ which came from comparing maximum allowable step sizes is removed. Instead, we enforce $\gamma \mu \tau \leq 1$, which gives us the weaker condition $\tau = \mathcal{O}(\frac{\sigma^2}{\epsilon \mu^2})$. Our condition on the overlap is then: $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\frac{\sigma^2}{\epsilon \mu^2}\})$. We see that this is similar to the condition obtained in \cite{mania2017perturbed} in their Hogwild! analysis, although we have the variance at the optimum $\sigma^2$ instead of a squared global bound on the gradient.

% Moreover, the paper in \cite{nguyen2018sgd} shows that for stochastic problems arising in machine learning such bound always holds in $\ref{SGDbounded}$. They also propose an alternative convergence analysis of SGD with diminishing learning rate regime, which results in more relaxed conditions than those in \cite{bottou2018optimization}, specifically their work extends the analysis of SGD to provide analysis of Hogwild! with diminishing step sizes and without the assumption on bounded gradients.

% \subsection{Convergence Analysis of Averaging Federated learning}
% Federated Averaging \cite{sahu2018convergence,doan2017convergence,wang2019adaptive} is stochastic algorithms by nature; in that, each step of these algorithms, only a fraction of the users are sampled to perform the update. Moreover, the local optimizer could be stochastic, e.g. SGD. It is well known that for stochastic methods in order to converge to a stationary point, a decreasing step-size is required. This is in contrast to the non-stochastic methods, e.g. gradient descent, that can find a stationary point with constant step size. In order to analyze the convergence behavior of such methods with constant step size, which is what is usually deployed in practice, we need to somehow control the dissimilarity among the local functions. This could be achieved through assuming IID, i.e. homogeneous, data among users. But we aim to generalize this idea to heterogeneous setting, which would better represent the federated learning.


% \subsection{Convergence Analysis of Hybrid system}

==> Section/05_Experiment.tex <==
\section{Experiment}
\label{sec:experiment}

Without loss of generality, we implement SGD and Hogwild! algorithms with constant step sizes. Moreover, it is sufficient to only consider our $k$-round asynchronous FL where the clients run SGD with constant step sizes because this is the most practical setup. We use Python and Tensorflow in our programming. 

\textcolor{red}{Ha to Nhuong: need to describe everything in detail. For example, how many samples in the training datasets. What is the configuration of clients and system. How do you implement Hogwild!, i.e., how to implement the memory lock for atomic reads and writes. What is the delay we introduce for atomic reads/ writes in the simulation.}

In this paper, we mainly focus on convex problem in machine learning, especially logistic regression problem with $\ell_{2}$ regularization.

The weight $w$ of the logistic function can be learned by minimizing the log-likelihood function $J$ (the logistic regression loss function) through gradient descent.
\begin{equation} \label{eq_logstic_reg}
    J = - \sum_{i}^N [ y_{i} \cdot \log (\sigma_i) + (1 - y_{i}) \cdot \log (1 - \sigma_i) ] + \frac{\lambda}{2}\norm{w}^{2},
\end{equation}
where $N$ is the number of training samples, $\lambda$ is regularization parameter, $\sigma$ is a sigmoid function with parameters weight $w$, bias value $b$ and input data $x$ defined as:
\begin{equation} \label{eq_sigmoid}
    \sigma(w, x, b) = \frac{1}{1 + e^{-(w^{\mathrm{T}}x + b)}}.
\end{equation}

\subsection{Simulation of SGD and Hogwild! and their comparison}
\label{subsec:hogwild_simu}

We consider the binary classification for digits $0$ and $1$ for MNIST dataset. The goal of this experiment is to study the behavior of Hogwild! and the limitation of delay variable $\tau$. \textcolor{red}{For simulating the atomic read and write operation, we partition the full model $w$ into $m$ parts and these parts are locked by synchronized lock to guarantee the atomic operation. Moreover, in order to simulate the delay of read and write operation, we define atomic read and write operation will take 2 milliseconds, 1 millisecond respectively.} The detail sett up of the experiments is described below:
\begin{table}[ht]
\caption{Hogwild! training parameters}
\label{tbl_hogwild}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & 1/$N$ &    \\
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
%Size of Dataset & ????&   \\

% \hline
Number of atomic writes & 50000 &                       \\
% \hline
Image size & 28x28   & grayscale                        \\
Data set records $N$ & 14867 &                          \\
% \hline
Number of threads $n$ & 1/3/5/10/15/20 &                  \\
% \hline
Number of masks $m$ & 14 &                               \\
% \hline
Epoch & 20 &                                            \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[hbt]
  \centering
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/04_hogwild_and_sgd_train_loss.PNG}
\caption{The training loss at the end of each epoch.}
\label{fig:hogwild_train_err}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/03_hogwild_and_sgd_train_duration.PNG}
\caption{Average training duration with different number of threads.}
\label{fig:hogwild_duation}
  \end{minipage}
\end{figure}

Figures~\ref{fig:hogwild_train_err} and \ref{fig:hogwild_duation} show the training error and speedup rate for training process using the Hogwild! algorithm. When n$\_$thread=1, Hogwild! is exactly SGD. As can be seen from Figure~\ref{fig:hogwild_train_err}, while the number of threads increases, the values of training error for all threads are nearly the same. It means that single thread SGD and Hogwild! with multiple threads have the same accuracy or training error. In contrast to Figure~\ref{fig:hogwild_train_err}, we see a significant decrease of training duration when the number of threads goes up. However, the number of joined threads needs to be reasonable due to the limit of max delay $\tau$ and the number of masks, which can reduce the performance of training process due to the effect of collision in atomic read and atomic write constraints. For example, when n$\_$thread=20, the duration increases instead of decreasing due to the effect of atomic read or write. 

\subsection{Simulation of our $k$-round asynchronous FL}
\label{subsec:kroundFL_simu}

In order to understand the behavior of the FL systems. We conduct the following experiments. 


\begin{table}[ht]
\caption{Federated Learning with different number of samples.}
\label{tbl_samples}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
Number of clients $n$ & 3 &                              \\
% \hline
Image size & 28x28   & grayscale                    \\
Train dataset records & 14867 &                          \\

% \hline
Number of samples $s$ & 10/50/100/500/1K/2K/\\ &2.5K/10K/15K &                  \\
% \hline
Number of round $r$ & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_sample_train_error.PNG}
\caption{FL with different number of samples.}
\label{fig:fl_sample}
\end{figure}

\vspace{0.2cm}
\noindent
\textbf{Varying the size of samples $s$ while fixing parameters $k,n$ and $\eta$:} The goal of this experiment is that $s$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). The detailed setup of this experiment for logistic regression problem is described in Table~\ref{tbl_samples}.

Figure~\ref{fig:fl_sample} reveals that when the number of samples $s=500$, we gain the highest accuracy. In addition, if we continue to increase the number of samples, the accuracy keeps nearly unchanged, i.e, large number of samples does not guarantee the improvement of accuracy.

\vspace{0.2cm}
\noindent
\textbf{Varying the number of clients $n$ while fixing parameters $k,s$ and $\eta$:} The goal of this experiment is that $n$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). \textcolor{red}{We choose the small stepsize for the simulation due to the fact that we need the large number of samples and clients to show that large number of clients can affect the train accuracy.} The detail parameters of this experiment are illustrated in Table~\ref{tbl_clients}.

\begin{table}[ht]
\caption{Federated Learning with different number of clients.}
\label{tbl_clients}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.00025 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
% \hline
Image size & 28x28   & grayscale                    \\
Data set records & 14867 &                          \\
% \hline
Number of clients $n$ & 5/10/20/30/40/50 &                  \\
Number of samples $s$ & 5000 &                  \\
% \hline
$k$-round & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_client.PNG}
\caption{FL with different number of clients.}
\label{fig:fl_client}
\end{figure}

Figure~\ref{fig:fl_client} shows that when number of client $n=30$, the training process gain the lowest train error, i.e, the largest accuracy while if $n$ continue to increase, the accuracy will dramatically decreases.

\vspace{0.2cm}
\noindent
\textbf{Varying the round parameter $k$ while fixing parameters $n,s$ and $\eta$:} The goal of this experiment is to verify the convergence rate of the system when $k$ increases. Table~\ref{tbl_k_round} defines the detail parameters of the experiment.


\begin{table}[ht]
\caption{Federated Learning with different number of $k$-round.}
\label{tbl_k_round}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.0001 &  fixed                         \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                    \\
% \hline
% \hline
Image size & 28x28   & grayscale                        \\
Data set records & 14867 &                              \\
% \hline
Number of clients $n$ & 3 &                                  \\
Number of samples $s$ & 1000 &                              \\
% \hline
Number of rounds & 5 &                                   \\
$k$-round & 1/2/3/4/5/6 & asyn-round of client                   \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_k_round.PNG}
\caption{FL with different number of $k$-round.}
\label{fig:fl_k_round}
\end{figure}

As can be seen from Figure~\ref{fig:fl_k_round}, when we change the $k$-round value from 1 to 2 and 3, the train error goes down dramatically. It means that asynchronous FL helps the model converge faster than the traditional FL. However, when we continue to increase the value $k$, the train error almost remains unchanged.


\textcolor{red}{\textbf{Important Note}:} From the implementation, we have the following observation: assume that there exists a good $k$-asynchronous FL, i.e., the clients always get a new model $w$ from the server before finishing all $k$ rounds of computation. Then for any $k'(>k)$-round asynchronous FL, it should include that good $k$-round asynchronous one. This fact leads to the important following result: the clients always get the new model $w$ before finishing all $k$ rounds rather than $k'$ rounds. In other words, $k'$ can be arbitrary large or the clients seem never be in \textit{waiting mode} as described in Figure~\ref{fig:framework_waiting}. Therefore, the designer only needs to find the optimal numbers $s$ and $n$ and can ignore the parameter $k$ by setting it  large. This allows the clients and server to work in a fully asynchronous mode. 


\subsection{Real applications of Federated learning}

\textbf{Text prediction on Android phone}: We can create an Android phone for chatting purpose. Based on the text content from client, we can used it for training a text prediction model. We can take reference from Google Keyboard application \cite{GoogleAIBlog,hard2018federated}.

\textbf{Diseases Detection based on daily activities}: Based on mobile phone, we can collect behavioral data from client, for example, sleep time, exercise habit, daily activities. Certain activities in daily life can reflect early signals of some diseases, so we can create a mode for detecting common diseases. For example, without enough sleep, people can suffer from seizure or mental disorders \cite{chen2019fedhealth}.

\textbf{Music recommendation engine:} which recommends music on an app for users. Specifically, we can predict emoji from text typed on a mobile keyboard and then recommends appropriate music for users \cite{ramaswamy2019federated}.

\textbf{Fraud detection model:} multiple banks could train a common powerful fraud detection model without sharing their sensitive customer data with each other through Federated Learning.


\textcolor{red}{https://hackernoon.com/a-beginners-guide-to-federated-learning-b29e29ba65cf}


\textbf{Technologies and Frameworks for Federated Learning
:} Some of the popular and recent Federated Learning frameworks include TensorFlow Federated, an open source framework by Google for experimenting with machine learning and other computations on decentralized data. PySyft is a open source library that is built on top of PyTorch for encrypted, privacy preserving deep learning. Federated AI Technology Enabler (FATE) is an open-source project initiated by Webank’s AI group to provide a secure computing framework to support the Federated AI ecosystem.

Several new startups such as S20.ai, Owkin, and Snips have emerged in this space creating new tools and enterprise solutions around Federated Learning and other secure computation techniques across different verticals

\textbf{Federated Learning is still in its early stages and faces numerous challenges with its design and deployment.
}
For instance, its feasibility is highly constrained by the capabilities of the edge devices to perform local training and inferencing. While this may not remain a major barrier to entry as most smartphones and IoT devices newly launched are equipped with GPUs or sufficient computing hardware to run powerful AI models. Today it’s still impossible to train a network without compromising device performance and user experience or compressing a model and resorting to a lower accuracy.

Local training of supervised models requires labeled data which isn’t available or difficult to produce in most cases. A good way to tackle this challenge is by defining the Federated Learning problem and designing data pipeline such that labels are captured in an implicit way, for example, user’s interactions, feedback on model responses based on certain actions taken or events triggered, etc.

In real world cases, model convergence time is higher in the Federated setup as compared to the traditional central training approach. There could be reliability issues where not all devices participate in the Federated Learning process due to connectivity issues, different app usage patterns and model training times, irregular or missed updates, etc. Federated Learning should be considered only when the size of the data and cost of aggregating from distributed sources is very high. inconsistent model versions across the clients does not affect the experience too much for a significant time window and the central model can converge with minimal client participation.

Finally, the mindset of centrally aggregating data and creating silos by large companies for competitive advantage would be a major challenge to drive the adoption of Federated Learning. Effective data protection policies and appropriate incentives and business models around decentralizing data can tackle these issues and develop the Federated AI ecosystem
















==> Section/08_Proposal_citations.tex <==
\section{Proposal Citations}
\label{sec:proposal_citations}

The detail list of papers in federated learning is illustrated in ~\cite{yang2019federated,tianli2019federated}.

Ref: https://arxiv.org/pdf/1902.04885.pdf

Ref: https://arxiv.org/pdf/1908.07873.pdf

\vspace{2mm}
\noindent
\textbf{Introduction of Federated Learning}

~\cite{konevcny2016federated} introduced the concept of federated learning in 2016. They used the android application (Google keyboard) to demonstrate the text prediction application.

~\cite{mcmahan} described the original federated learning for deep learning task. Specifically, the server will take average of all models from clients.

~\cite{tianli2019hetero} introduced FedProx, which makes a small modification to the~\cite{mcmahan} method to help ensure convergence, both theoretically and in practice. FedProx can also be interpreted as a generalized, reparameterized version of FedAvg that has practical ramifications in the context of accounting for systems heterogeneity across devices.

\vspace{2mm}
\noindent
\textbf{Architecture of Federated Learning}

\begin{figure}[ht]
  \centering
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{Figures/horizon.PNG}
\caption{Horizontal architecture of FL.}
\label{fig:horizontal_fl}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{Figures/vertical.PNG}
\caption{Vertical architecture of FL.}
\label{fig:vertical_fl}
  \end{minipage}
\end{figure}

\textbf{Horizontal Federated Learning or sample-based federated learning} \cite{mcmahan,tianli2019hetero,bonawitz2019towards,konevcny2016federated,konevcny2016federated_com}, is applied in the scenarios that local data sets in clients share the same feature space but different in samples. A typical architecture for a horizontal federated learning system is shown in Figure ~\ref{fig:horizontal_fl}. In this system, $k$ clients with the same data structure collaboratively train independently global model with the help of a parameter server. In addition, a typical assumption \cite{phong2018privacy} is that the participants are honest while the server is honest-but-curious, hence no leak information from any participants to other participants and the server is allowed.

\textbf{Vertical federated learning or feature-based federated learning} \cite{nock2018entity,yang2019federated,hardy2017private} is applied in cases that data sets in client sides share the same sample space but differ in feature space (shown in Figure~$\ref{fig:vertical_fl}$a). It is the process of aggregating these different features and computing the training loss and gradients in a privacy-preserving manner to build a model with data from parties collaboratively. In addition, a vertical federated learning system typically assumes honest-but-curious participants. In the security perspective, it means that the adversary can only learn data from the corrupted clients but not data from other clients or from server. Recently, there are a lot of researches which have proved that FL can work very well with various machine learning models (for example, logistic regression, tree structure and neural network) \cite{gascon2016secure,karr2009privacy,vaidya2002privacy,wan2007privacy}.

\textbf{Federated Transfer Learning} \cite{pan2009survey} can be used to the scenarios that the data sets in client sides are different from in both sample spaces and feature space, so transfer learning technique can handle the problem of lacking data (few samples and features) or weak supervision (few labels). We can distinguish the major difference between vertical FL and federated transfer learning is that federated transfer learning can exchange models among clients, which is not seen in vertical FL (shown in Figure~$\ref{fig:vertical_fl}$a,b). However, the set of overlapped data from clients could be small (for example the different businesses in reality) and make federated transfer learning less attractive and effective. Interestingly, the paper in \cite{yang2018secureftl} proposes a possible solution to these above challenges by exchanging the models using homomorphic encryption among clients, which leverages the transfer learning technique proposed by \cite{pan2009survey} to provide solution for training FL with the sample and feature space under a data federation and privacy-preserving constraints.

\vspace{2mm}
\noindent
\textbf{Privacy-preserving and Security under Federated Learning}

\textbf{Privacy} is one of the essential properties of federated learning. This requires security models and analysis to provide meaningful privacy guarantees.

Secure Multi-party Computation (SMC) \cite{wenliang,payman,dan} naturally involved multiple parties, and provide security proof in a well-defined simulation framework to guarantee complete zero knowledge, that is, each party knows nothing except its input and output. Zero knowledge is very desirable, but this desired property usually requires complicated computation protocols and may not be achieved efficiently.


Differential Privacy \cite{cynthia,dwork2014algorithmic,abadi2016deep,geyer2017differentially,mcmahan2017learning} involves in adding noise to the data, or using generalization methods to obscure certain sensitive attributes until the third party cannot distinguish the individual, thereby making the data impossible to be restore to protect user privacy. However, the root of these methods still require that the data are transmitted elsewhere and these work usually involve a trade-off between accuracy and privacy.

Homomorphic Encryption \cite{rivest,qingchen,abbas} is also adopted to protect user data privacy through parameter exchange under the encryption mechanism during machine learning. Unlike differential privacy protection, the data and the model itself are not transmitted, nor can they be guessed by the other party’s data. Therefore, there is little possibility of leakage at the raw data level. Recent works adopted homomorphic encryption for centralizing and training data on cloud.

\textbf{Model-poisoning attacks in Federated Learning}

~\cite{nasr2019comprehensive} shows how adversarial participants, in the federated learning setting, can successfully run active membership inference attacks against other participants, even when the global model achieves high prediction accuracies.

~\cite{eugene} argued that federated learning is fundamentally vulnerable to backdoor attacks. First, when training with millions of participants (\textit{the attackers can directly influence the weights of the global model}), it is impossible to ensure that none of them are malicious. Second, federated learning by design has no visibility into what these participants are doing locally (\textit{the attackers can train the global model in any way that benefits poisoning}), and “secure aggregation” provably prevents anyone from auditing participants’ updates to the joint model. Existing defenses against data poisoning cannot be used for federated learning because they all require access to the training data.

~\cite{arjun} exploited the lack of transparency in the agent updates, and explore the possibility of an adversary controlling a small number of malicious agents performing a model poisoning attack. The adversary’s objective is to cause the jointly trained global model to misclassify a set of chosen inputs with high confidence, i.e., it seeks to poison the global model in a targeted manner. Since the attack is targeted, the adversary also attempts to ensure that the global model converges to a point with good performance on the test or validation data. Moreover, they focus on an adversary which directly performs model poisoning instead of data poisoning \cite{battista,huang} as the agents’ data is never shared with the server.


\vspace{2mm}
\noindent
\textbf{Asynchronous SGD training technique}~\cite{zinkevich2009slow,lian2015asynchronous,lian2017asynchronous,zheng2017asynchronous,meng2017asynchronous,stich2018local,shi2019distributed} is widely used in traditional distributed stochastic gradient descent (SGD). Typically, asynchronous SGD converges faster than synchronous SGD. However, classic asynchronous SGD directly sends gradients to the server after each local update, which is not practical for edge devices (such as mobile or IoT devices) due to the unreliable and slow communication.

% ~\cite{congxie2019} \textcolor{red}{proposed a new asynchronous federated optimization algorithm and proved that the proposed approach has near-linear convergence to a global optimum, for both strongly and non-strongly convex problems. However, their proof is not based on Hogwild! scheme}.

\vspace{2mm}
\noindent
\textbf{Communication Cost in Federated Learning}

In order to reduce communication in such a setting, two key aspects to consider are: (1) reducing the total number of communication rounds, or (2) reducing the size of transmitted messages at each round.

Local updating methods can reduce the total number of communication rounds \cite{jaggi2014communication,zhang2015deep,smith2016cocoa}.

Model compression schemes such as sparsification, subsampling, quantization, compression algorithms can significantly reduce the size of messages communicated at each round \cite{chen2015compressing,han2015deep_compression,konevcny2016federated_com,jacob2018quantization,caldas2018expanding, sattler2019robust}.

Decentralized training \cite{lian2017can,he2018cola,lalitha2019decentralized} and hierarchical communication \cite{lin2018don,liu2019edge} are proposed by to reduce the communication and computation from the central server. Specifically, the intermediate servers will aggregate the updates from clients and then the central server only aggregate updates from edge servers.

\vspace{2mm}
\noindent
\textbf{Fault Tolerance in Federated Learning system:}
The federated learning system in reality also needs to address not only high communication costs but also stragglers and fault tolerance issues~\cite{tandon2017gradient,bonawitz2019towards,yu2019distributed,chen2019efficient}.


\vspace{2mm}
\noindent
\textbf{Benchmark tools for federated learning system}

LEAF \cite{caldas2018leaf} is an open-source, modular benchmarking framework for learning in federated settings. Source code: https://leaf.cmu.edu/

TensorFlow Federated \cite{tensorflow_federated} is an open-source framework for machine learning and other computations on decentralized data, which is released by Tensorflow team. Source code: https://github.com/tensorflow/federated

\vspace{2mm}
\noindent
\textbf{Dataset}

MNIST~\cite{lecun-mnisthandwrittendigit-2010}

FashionMNIST~\cite{xiao2017fashion}

CIFAR-10~\cite{Krizhevskycifar10}

Netflix Prize dataset~\cite{Bennett07thenetflix}

UCI Smartphone~\cite{reyes2012human}



==> Section/09_Experiments_full.tex <==
\section{Experiments for asynchronous SGD | Hogwild! and asynchronous Federated Learning}

\subsection{Experiment problem}
The weight $w$ of the logistic function can be learned by minimizing the log-likelihood function $J$ (the logistic regression loss function)
\begin{equation} \label{eq_logstic_reg2}
    J = - \sum_{i}^N [ y_{i} \cdot \log (\sigma_i) + (1 - y_{i}) \cdot \log (1 - \sigma_i) ] + \frac{\lambda}{2}||\norm{w}||^{2},
\end{equation}
where $N$ is the number of training samples, $\lambda$ is regularization parameter, $\sigma$ is a sigmoid function with parameters weight $w$, bias value $b$ and input data $x$ defined as:
\begin{equation} \label{eq_sigmoid2}
    \sigma(w, x, b) = \frac{1}{1 + e^{-(w^{\mathrm{T}}x + b)}}.
\end{equation}

\subsection{Experiments for Hogwild!} \footnote{The experiments for Hogwild! solved the convex problem.}
For comparing the convergence of Hogwild! for constant and diminishing stepsize, there are some notes in the setting:

\begin{itemize}
    \item {use a reasonable value of $\lambda$.}
    
    \item{use a small value of $D$. For example, we use $D = 7$ for MNIST and Fashion MNIST and $D=8$ for CIFAR10 dataset.}
    
    \item {small value of constant stepsize.}
    
\end{itemize}

\begin{table}[tb]
\caption{Hogwild! training parameters}
\label{tbl_hogwild_exp}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & $0.1/0.15/0.05$ &    \\
Constant learning rate $\eta$ & 0.001 &                         \\ 
% \hline
Data set & MNIST &                \\

% \hline
Number of atomic writes & 12500 &                       \\
% \hline
Image size & 28x28   & grayscale                        \\
Batch size $b$ & 10 &                                   \\
% \hline
Number of threads $n$ & 3 &                             \\
% \hline
Number of masks $m$ & 7 &                               \\
% \hline
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Table~\ref{tbl_hogwild_exp} illustrates the detailed parameters used for conducting experiments for Hogwild! The goal of this experiments is to see the convergence of Hogwild! on different datasets. The results are described below:
\begin{figure}[ht]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x10_500x25_stepsize_0x001.png}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\label{fig:hogwild_mnist_01_0}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x15_500x25_stepsize_0x001.png}
\label{fig:hogwild_mnist_01_1}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x05_500x25_stepsize_0x001.png}
\label{fig:hogwild_mnist_01_2}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x10_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_0}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x15_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_1}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x05_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_2}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x10_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_0}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x15_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_1}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x05_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_2}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}


\begin{table}[h]
\caption{Asynchronous Federated Learning (FL) parameters}
\label{tbl_FL_mnist_k_1}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & $0.1$ &    \\
Constant learning rate $\eta$ & 0.001 &                         \\ 
% \hline
Data set & MNIST & Digit 4 and 5               \\
Data set & Fashion MNIST & Coat and Sandal               \\
%Size of Dataset & ????&   \\

% \hline
Number of atomic writes & 12500 &                       \\
% \hline
Image size & 28x28x1   &                         \\
Batch size $b$ & 10 &                                   \\
Asynchronous round $k$ & 1/2 &                          \\
% \hline
Number of client $n$ & 1 server and 2 clients &                  \\
% \hline
Number of masks $m$ & 7 &                               \\
% \hline
% Epoch & 20 &                                            \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Table~\ref{tbl_FL_mnist_k_1} illustrates the detailed parameters used for conducting experiments for asynchronous FL. The goal of this experiments is to see the accuracy of traditional FL and asynchronous FL with different communication round. The communication round $k$ means the number of times clients and server exchange their gradients (models) values and less value of $k$ means better communication costs. The results are described in Table~\ref{tbl_FL_mnist_k_1_result},\ref{tbl_FL_famnist_k_1_result} below:
\begin{table}[h]
\caption{Asynchronous Federated Learning result for MNIST}
\label{tbl_FL_mnist_k_1_result}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Experiment & Test Accuracy (\%) & Communication round\footnote{Number of rounds clients and server exchange their models.} \\ [0.5ex]
\midrule
Traditional FL\footnote{Traditional FL uses a constant stepsize.}  
& $93.717$ &   5       \\
Traditional FL   & $93.775$ &   4                   \\
Traditional FL   & $94.101$ &   3                   \\
Traditional FL   & $88.951$ &   2                   \\
Asynchronous FL ($k=1$)  & $96.496$  &   2          \\
Asynchronous FL ($k=2$)  & $95.904$  &   2          \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[h]
\caption{Asynchronous Federated Learning result for FashionMNIST}
\label{tbl_FL_famnist_k_1_result}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Experiment & Test Accuracy (\%) & Communication round \\ [0.5ex]
\midrule

Traditional FL\footnote{Traditional FL uses a constant stepsize.}   
& $87.135$ &   5           \\

Traditional FL   & $87.435$ &   4           \\
Traditional FL   & $89.005$ &   3           \\
Traditional FL   & $92.727$ &   2           \\
Asynchronous FL ($k=1$)  & $97.675$  &   2          \\
Asynchronous FL ($k=2$)  & $94.145$  &   2          \\


\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\subsection{Experiments for asynchronous Federated Learning}

\subsection{Experiments for Differential Privacy - Federated Learning}

TODO: Experiments Description & Experiments Results

% Strongly convex case

% Plain convex case

% Non convex case

==> Section/10_DP.tex <==
%\section{Main DP Theorem}
%\label{sec:theory}
%\subsection{Differential privacy} \label{sec:DP}

%Differential privacy \citep{dwork2006calibrating, dwork2011firm,dwork2014algorithmic,dwork2006our} defines privacy guarantees for algorithms on databases, in our case a client's sequence of mini-batch gradient computations on his/her training data set. The guarantee quantifies into what extent the output  of a client (the collection of updates communicated to the server) can be used to differentiate among two adjacent training data sets $d$ and $d'$ (i.e., where one set has one extra element compared to the other set).

%\begin{defn} \label{defDP} A randomized mechanism ${\cal M}: D \rightarrow R$ is $(\epsilon, \delta)$-differentially private if for any adjacent $d$ and $d'$ in $D$ and for any subset $S\subseteq R$ of outputs,
%$$ Pr[{\cal M}(d)\in S]\leq e^{\epsilon} Pr[{\cal M}(d')\in S] + \delta.$$
%\end{defn}



%Note however, Theorem \ref{thmsc2} on the convergence rate for strong convex problems 
%does not hold for the adapted version. Nevertheless experiments in Section \ref{sec:experiment} show that copying over the suggested step size sequences and sample size sequences lead to proper convergence and accuracy. 

%\begin{algorithm}[!t]
%\caption{Client$_c$ -- Local Model with DP}
%\label{alg:DP}
%
%\begin{algorithmic}[1]
%\Procedure{MainClientDP}{$\mathcal{D}_c$} 
%\State $i=0$, $\hat{w}=\hat{w}_{c,0,0}$ 
% 
%\While{\textbf{True}}
%    \State $h=0$, $U=0$ 
%    \While{$h< s_{i,c}$}
%    
%              \State $t_{glob}= s_0+\ldots+s_{i} - (s_{i,c}-h)-1$
%       \State $t_{delay} = s_{k}+\ldots+s_{i} - (s_{i,c}-h) $
%       \State {\bf while} 
%       $\tau(t_{glob}) = t_{delay}$ 
%       {\bf do} nothing {\bf end while}
% 
%        
%        \State Sample uniformly at random $\xi$ from $\mathcal{D}_c$ 
%        
%        \State $g = \nabla f(\hat{w}, \xi)$ 
%        
%        \State $g = g / \max \{1, \|g\|/C\ \}$ \Comment{NEW: Clip gradient}
%        
%        \State ${U} = {U} + g$  
%        
%        \State Update model $w = \hat{w} - \bar{\eta}_{i} \cdot g$ \Comment{$w$ represents $ w_{c,i,h+1}$} 
%         \State Update model $\hat{w} = w$  
%
%        \State $h$++
%    \EndWhile
%    
%    \State $n\leftarrow N(0,C^2 \sigma_i^2\textbf{I})$ \Comment{NEW: Draw batch noise}
%    \State $\hat{w}= \hat{w}+\bar{\eta}_i\cdot n, U=U+n$ \Comment{NEW: Include batch noise} 
%    
%    \State Send $(i,c, U)$ to the Server. 
%    \State $i$++
%\EndWhile
%   
%\EndProcedure   
%
%\end{algorithmic}
%\end{algorithm}



%In order to obtain privacy guarantees, we want to apply the DP theory from \citep{abadi2016deep} for (diminishing) step size sequence $\{\bar{\eta}_i\}$ and increasing sample size sequence $\{s_{i}\}$. 
%Next theorems show how this is done 



%\vspace{3mm}
%
%\noindent
%\textbf{Utility $\sigma$:} 
%In the DP approach, the utility which we wish to achieve measures accuracy. We aim at sufficient high accuracy. We cannot write out this utility function in closed form. In Section \ref{sec:experiment} we simulate for various $\sigma$ the accuracy achieved by a global optimal model generated without adding any noise during any of the rounds except for the very last round. This upper bounds the accuracy that can be achieved if noise were added at the end of each round as in DP-SGD. The result is a utility graph which can be used to upper bound $\sigma$ beyond which the accuracy will certainly suffer too much. As the simulations show, a smaller clipping constant $C$ allows larger $\sigma$ (hence, better privacy) albeit at slower convergence (that is, larger $K$). 


%The simulations in the next section use smaller data sets (relatively small $N$) and are therefore based on parameters that satisfy the exact theorem's constraints (\ref{treq1}, \ref{treq2}, \ref{treq3}, \ref{sigeps}). 
%The introduction explains 

%Another equivalent formulation is
%\begin{equation}
%N \geq  \frac{\gamma}{2} \frac{\sigma^2 \theta^2 }{\epsilon + \ln(1/\delta)} \cdot (K/N) \cdot \bar{s}, \label{treqN}
%\end{equation}
%which shows that $N$ should be a factor larger than the number of local gradient computations across all rounds measured in epochs (of size $N$) times the mean mini-batch/sample size. In practice this generally means that (\ref{treqN}) is not constraining since $N$ is much larger than the lower bound in (\ref{treqN}).

%Into what extent is this upper bound restrictive?

%%%%%%%%%%%%%%%
%[TO DO: thorough edit, more smooth; more words on utility; modeling N for features -- distribution which groups data into N labels and we select at random (some probability) a label -- this is translated into an actual data from the group -- etc. -- DP holds]
%[Move small N to appendix]
%%%%%%%%%%%%%%%%%%%

%\textbf{Insensitivity to $T$:} The above discussions show that for large enough $N$ we only need to make sure that (\ref{sigeps}) is satisfied:
%$$ \sigma = \sqrt{2(\epsilon + \ln(1/\delta)) /\epsilon}.$$
%The resulting DP guarantee is remarkably {\em insensitive to increasing the number $T$ of rounds} (which makes $\bar{s}=K/T$ even smaller and (\ref{treqN}) easier to satisfy). More rounds does mean more privacy leakage as more and more information about the local data set (in the form of updates $U$) becomes available. The added Gaussian noise is sufficient not to violate the DP guarantee up to the moment $T$ is maxed out at $T=K$. This allows us to freely choose a 'best' total number of rounds in the sense that on one hand we want to minimize round communication and on the other hand sufficient round communication is needed in order to channel information about one's local data set to the other clients. The latter is especially important when local data sets are more heterogeneous than iid. 

%Notice that this is a significant improvement over \citep{abadi2016deep} where the lower bound on $\sigma$ scales with $\sqrt{T}$, hence, $T$ must be small enough and their constant sample size large enough. The reason for this is that  \citep{abadi2016deep} essentially stops at Theorem \ref{thm1} where the lower bound on $\sigma$ also seems to scale with $\sqrt{T}$; they did not think about having ``constants'' $c_0$ and $c_1$ depend on parameters such as $T$, $K$, and $N$.

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%\textbf{Small $N$:} 
%For small $N$ where (\ref{treqN}) becomes restrictive, we want to understand into what extent we can guarantee DP. As a trick, we may attempt to artificially enlarge the local data set by creating a dummy entry to each data element:
%$$
%d_{new} = \{ (x,j) \ : \ x\in d, 1\leq j\leq k\},
%$$
%where the dummy entry $j$ is neglected when evaluating  gradients.
%This makes $|d_{new}|=k|d|=kN$ and we can plug this large data set size into (\ref{treqN}) in order to satisfy the bound. However, this does not come for free because an adversary knows that trying to figuring out whether $x\in d$ is equivalent to deciding whether the whole cluster $\{(x,j)\}_{j=1}^k\subseteq d_{new}$. This means that we need to consider the DP guarantee for extended data sets $d_{new}$ and $d'_{new}$ that differ in one cluster of size $k$. If we recursively apply the bound of Definition \ref{defDP} $k$ times in a straightforward manner, then
%$$ Pr[{\cal M}(d_{new})\in S]\leq e^{k\epsilon} Pr[{\cal M}(d'_{new})\in S] + \frac{e^{k\epsilon}-1}{e^\epsilon -1}\delta.$$
%This shows the weaker DP guarantee, in effect, $\epsilon$ is a factor $k$ larger. If we want to maintain the original DP guarantee, then we should start with $\epsilon/k$ in (\ref{sigeps}) and this makes $\sigma$ a factor $\approx \sqrt{k}$ larger. It turns out that this corresponds to the other case in Theorem \ref{thm1} for $c(c_1)<1/(\hat{\rho} x)$: This makes $c_0$ smaller and the lower bound on $\sigma$ larger. A calculation for a constant sample size sequence ($s_i=\hat{s}$) shows that this other case leads to an $\Theta(\sqrt{k})$ larger lower bound on $\sigma$ confirming the conclusion above. The advantage of (moderately) large data sets is the insensitivity to $T$ (and $\bar{s}$) as discussed above.
%
%
%\textbf{$N$'s interpretation:} 
%Suppose each local data set comes from a similar source, e.g., they all have clusters of images corresponding to certain labels like cars, boats, planes, etc. Clearly, anyone knows that a client's local data set contains these classes of pictures. The client wishes to keep identifying information private such as the number plates on the cars, or the harbour where the boat is pictured. This type of information concerns small features which the global model does not attempt to learn (and later reveal). From this perspective $N$ represents the number of images in the local data set with different small features (which one wishes to keep private). Features that represent coarser classification information and are repeated over multiple images in the local data set effectively correspond to a DP guarantee for a smaller $N$. This means that the lower bound in (\ref{treqN}) can be interpreted as the minimal $N$ for which the "corresponding features" remain $(\epsilon,\delta)$-DP. 
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%---





%Discussion constraints: first two generally immediately satisfied because ..

%utility graph constrains the last one -- the lower bound is strong as it allows smaller eps than previously reported -- satisfying our aim of truly small closer to 0 eps values

%discuss that case 1 leads to a smaller lower bound than case 2 - thus we prefer to set parameters so that we are in case 1

%choose $\delta$ always $1/N$ ..

%second last constraint generally satisfied for large N compared to mean sample sizes: we cannot simulate very large data sets, so we do get constrained here

%Discussion  on N ... essentially in our interpretation N is often smaller than the true N ...

%So, in practice with proper intuition we have 
%$$ \sigma = \sqrt{2\ln(1/\delta)/\epsilon}, \mbox{ i.e. } 
%\epsilon = 2\ln(1/\delta)/\sigma^2.$$
%as small as possible for best accuracy, hence, we need
%$$ \sigma \leq \sqrt{ \frac{2 \ln(1/\delta)}{\gamma \theta^2 \cdot (K/N) \cdot (\bar{s}/N)}},$$
%where $\gamma$ is also a function of $\sigma$ (also notice that it depends on $\epsilon$ in $\bar{\alpha}$ which is a function of $\sigma$).
%This is the expected upper bound we usually see in DP theory.

%If we can realize small $\epsilon$, then $\gamma$ is closer to $2$, hence, the bound on $\sigma$ will be determined by the utility graph rather than this inequality if $K/N$ can be compensated by $\bar{s}/N$, i.e., we want $\bar{s}$ a factor smaller than $N^2/K$ showing that $K$ measured in epochs is at most a factor smaller than $N$ -- for large data sets this is always the case.

%the upper bound also shows that $\bar{s}$ must be bounded by a factor smaller than $N$ otherwise we cannot have larger $\sigma$ or equivalently smaller $\epsilon$.

%\begin{equation}
%\gamma \theta^2 \cdot \frac{K}{N} \cdot \frac{\bar{s}}{N}  \leq \epsilon \leq \gamma  h(\sigma)\cdot \frac{K}{N}
%\end{equation}
%and 
%\begin{equation}
%\bar{s} \leq \frac{g(\sqrt{2\ln(1/\delta)/\epsilon})}{\theta} \cdot N.
%\end{equation}

%\begin{equation} \sigma \geq \sqrt{2\ln(1/\delta)/\epsilon}. \nonumber
%\end{equation}

%=======================




%\subsection{Asynchronous Distributed SGD} \label{sec:ADSGD}

%\textbf{TODO:} Add the details of Asynchronous Distributed SGD here

%\input{Section/12_DP_RelatedWork}

==> Section/11_Calculator.tex <==

\subsection{DP Calculator}
% In this section, we introduce DP-calculators which search for smallest possible value of epsilon, delta and sigma given the dataset size $N_c$, increasing sequence of sample size $s_{i,c} = N_cq(i+m)^p$, initial sample size $s$ and number of epochs $K$.



% In the appendix, we show a lot of examples about computing delta value and this is also the way how we implement the delta-calculator which is described in the following algorithm:

%  \begin{algorithm}[ht]
% \caption{Delta calculator}
% \label{Delta calculator}
% \begin{algorithmic}[1]

%     \State {\bf Input:} $p \in [0,1],\sigma, N_c, r_0, \epsilon,K,s_{0,c}$
%     \State {\bf Initialize:} $\alpha = r_0/sigma, \gamma = 0, \gamma_{new} = \infty$

%     \While{$ \abs{\gamma_{new} - \gamma > 0.01 \times  \gamma} $}
%         \State $r = calculate\_r(r_0,\sigma)$
%         \If {$\gamma_{new} != \infty$} 
%             $\gamma = \gamma_{new}$
%         \EndIf
%         \State $uq_1 = compute\_q\_from\_K\_star(r_0,\sigma,p,\gamma,K)$
%         \State $uq_2 = compute\_q\_from\_K\_minus(p,\alpha,\gamma,r,\epsilon,K)$
%         \State $q = uq_1$ if $uq_1 < uq_2$, otherwise $q = uq_2$
%         \State $s = q \times N_c$
%         \State $m = compute\_m(N_c,q,p,s_{0,c})$
%         \State $T = ceil(compute\_T(p,K,q))$
%         \State $\gamma_{new} = m/T$
%     \EndWhile
%     \State $\gamma = \gamma_{new}$
%     \State $\delta = compute\_delta(eps,m,T,r_0,sigma)$
%     \State \Return delta,s,m,T,q

% \end{algorithmic}
% \end{algorithm}

% We use the delta calculator to find "good settings" in which delta is "small" enough (we assumed $delta < 0.01 \times N_c$ is a good result). However, we clearly notice that there is a trade-off between sigma, epsilon and delta value. Therefore, we come up with the sigma calculator which computes the smallest possible sigma for each hyper-parameter setting. Moreover, by running the delta calculator, we also get the increasing sequence size $s_{i,c}$ which is used in the sigma calculator.

% In theorem 6, we need K to be less than both $K^*$ and $K^-$. Therefore, we compute the upper bound of q: $uq_1,uq_2$ such that $K \leq K^*$ and $K^-$, respectively. After that, we choose the smaller upper bound to be the value of q (line 9). Then, we can easily compute the values of $s,m,T$ using the $compute_m$ and $compute_T$ functions (The detail is showed in the examples in appendix). Finally, we compute the new $\gamma = m/T$ and repeat until $\gamma$ is converged to at least two digits after the decimal point. Up till now, we assumed that $\gamma$ will converge if $\eps$ and $N_c$ is large enough. Finally, when we got all the components, we can compute the value of $\delta$ using the following inequality:
% \[\sigma \leq \sqrt{\frac{2\ln (1/\delta)}{\epsilon}}
%  \frac{(1+\gamma)^{2+3p}}{\sqrt{1-\alpha}}.\]

% % The sigma calculator which is implemented based on the \textbf{theorem 4} as follows:
% After we get the increasing sample size sequence, we use sigma calculator to find the smallest possible sigma in order to achieve the highest possible accuracy. 
% % The detail of sigma calculator is described in Algorithm 3.
% % \begin{algorithm}[
% % \caption{}
% % \label{Sigma calculator (Theorem 4)}
% % \begin{algorithmic}[1]

% % \end{algorithmic}
% % \end{algorithm}

% \begin{algorithm}
% \caption{Sigma calculator Part 1(Theorem 4)}
% \label{Sigma calculator Part 1(Theorem 4)}
% \begin{algorithmic}[1]
% \State {\bf Input:} $q,m,p \in [0,1],T,\delta,N_c,\epsilon,K$
%   \State {\bf Initialize:} \\ 
%   $B = 1/(1+p)\times pow((\sqrt{3}-1)/2 \times (2\times p+1),(1+p)/(1+2*p))$ \\
%   $A = B* pow(1+m/T,(3+4*p) \times (1+p)/(1+2*p))$ \\
%   $C_1 = pow(\epsilon,(1+p)/(1+2 \times p)) \times pow(q,-1/(1+2 \times p))$ \\
%   $K^- = B*C_1,K^+ = A*C_1, \sigma_{base} = 1.137$ \\
%     $\sigma_{smallest} = \infty$ \\
%     $diff = K^* = -\infty$
%     \For{$i=0,1,2,\dotsc, 20000$ } 
%     \State $\sigma = round(i*0.001 + \sigma_{base},3)$
%     \State $\gamma = m/T$
%     \State $r_0 = compute\_r0\_from\_K\_star(K,p,q,\sigma,\gamma)$
%     \State Calculate $u_0, u_1$ and check whether $u_0,u_1$ and $r_0$ are valid or not ($u_0,u_1 < 1, r_0 < 1/e$)
%     % \State $K^* = compute\_K\_star(r_0,\sigma,p,\gamma,q)$
%     \State $C_2 = \sqrt{2\times \log(1/delta)/\epsilon} \times pow(1+m/T,2+3*p) / \sqrt{1-r_0/sigma}$
    
% \algstore{bkbreak}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{Sigma calculator Part 2(Theorem 4)}
% \label{Sigma calculator Part 2(Theorem 4)}
% \begin{algorithmic}[1]
% \algrestore{bkbreak}
%     \If{$K <= K^-$}
%         \State $ diff = \sigma - C_2$
%     \EndIf
%     \If{$K >= K^+$}
%         \State $diff = \sigma - pow(K/K^+,(1+2\times p)/(2+2\times p))\times1.21\times C_2$
%     \EndIf
%     \If{$diff > 0$ and $\sigma_{smallest} > \sigma $}
%         \State $\sigma_{smallest} = \sigma$
%         \State Break
%     \EndIf
%     \EndFor
%     \State \Return $\sigma_{smallest}$
% \end{algorithmic}
% \end{algorithm}

% In this algorithm, we find $r_0$ such that $K = K^*$ and this is the smallest possible value of $r_0$ we can use. Surprisingly, our experiments show that we can even achieve $(eps,delta) = (0.4,2\times 10^{-6})$ for large datasets ($N_c = 500000$) with acceptable noise and training epochs: $\sigma = 11.675, K = 500$. We also experiment on various of dataset size and p to see how the value of sigma changes according to epsilon and delta.

% \begin{figure}
%   \centering
%   \subfloat[$N_c=10000,p=0.25$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_10000_p_25.png}\label{fig:async_fl_dp_1}}
%   \hfill
%   \subfloat[$N_c=10000,p=0.5$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_10000_p_50.png}\label{fig:async_fl_dp_2}}
%   \vskip\baselineskip
%   \subfloat[$N_c=10000,p=0.75$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_10000_p_75.png}\label{fig:async_fl_dp_3}}
%   \hfill
%   \subfloat[$N_c=10000,p=1$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_10000_p_100.png}\label{fig:async_fl_dp_4}}
%   \caption{Differential private sigma calculator with different p values}
%   \label{fig:async_fl_dp_01}
% \end{figure}

% \begin{figure*}
%   \centering
%   \subfloat[$N_c=10000,p=1$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_10000_p_100.png}\label{fig:async_fl_dp_5}}
%   \hfill
%   \subfloat[$N_c=50000,p=1$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_50000_p_100.png}\label{fig:async_fl_dp_6}}
%   \vskip\baselineskip
%   \subfloat[$N_c=100000,p=1$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_100000_p_100.png}\label{fig:async_fl_dp_7}}
%   \hfill
%   \subfloat[$N_c=500000,p=1$]{\includegraphics[width=0.5\textwidth]{Experiments/Calculator/Nc_500000_p_100.png}\label{fig:async_fl_dp_8}}
%   \caption{Differential private sigma calculator with different $N_c$ values}
%   \label{fig:async_fl_dp_02}
% \end{figure*}



==> Section/12_DP_RelatedWork.tex <==
\subsection{Related work}

Privacy-preserving in machine learning and deep learning has became a hot topic and received a lot of attractions. In order to prevent the data leakage from the inference attacks such as deep leakage machine learning attack
\citep{ligengzhu201deepleakage}, membership inference attack
\citep{shokri2017membership},..., a lot of privacy-preserving methods has been proposed
\citep{abadi2016deep,abhishek2018privateFL,mohammad2020privateFL,stacey2018privateFL,meng2020privateFL,robin2017privateFL,mcMahan2018privateFL,nicolas2018privateFL} .

$(\epsilon,\delta)$-Differential Privacy ($(\epsilon,\delta)$-DP) \citep{dwork2014algorithmic} is one of the most popular and powerful methods giving privacy. It provides a lot of privacy-preserving mechanisms which are compatible with most of machine learning, deep learning training algorithm such as Gaussian Mechanism, Laplace Mechanism,...
However, there is a trade-off between privacy budget $(\epsilon,\delta)$ and the performance of the machine learning model. In other words, if we have the smaller privacy budget $(\epsilon,\delta)$, then the performance of the machine learning model will be dropped as well. 

There are many existing privacy-preserving solutions utilize techniques for federated learning such as: Local Differential Privacy (LDP) \citep{abhishek2018privateFL,mohammad2020privateFL,stacey2018privateFL,meng2020privateFL}, Central Differential Privacy (CDP)\citep{mohammad2020privateFL,robin2017privateFL,mcMahan2018privateFL,nicolas2018privateFL}. In LDP, the noise required by DP is computed locally for each clients and it is added to the updates before sending to the server. In CDP, a \textbf{trusted} aggregate server is required to aggregate client's trained model's updates because the noise is only computed by this server and added to the global model hold by this server. However, most of the cited papers mentioned above need a very big privacy budget to achieve a similar performance compared with the non-DP setting. For example, in LDP based approach, for $10\%$ deduction in accuracy, \citep{abhishek2018privateFL,mohammad2020privateFL} needs $\epsilon = 500,\epsilon = 10.7$ respectively, and \citep{stacey2018privateFL,meng2020privateFL} used $\epsilon = 0.5$ as their best example for the smallest privacy budget. On the other hand, in CDP based approach, \citep{mohammad2020privateFL,robin2017privateFL,mcMahan2018privateFL} requires respectively $\epsilon = 8.1,\epsilon = 8,\epsilon = 2.038$ in order to achieve the closet accuracy to the non-DP setting.

Therefore, in this paper, we try to minimize the value of the privacy budget $(\epsilon,\delta)$ to be as small as possible without having the accuracy dropped down too much.

%TODO: MNIST hyperparameters setting comparison between DPSGD and our method. (done)
%TODO: explain in text exactly how our theory applies to their situation and what our theory predicts and how this compares to what they have chosen for the sigmas

In \cite{dwork2014algorithmic}, the authors use Principal Component Analysis (PCA) projections to improve both the training performance and model's accuracy. More specifically, they apply  differentially private PCA algorithm in \cite{Dwork2014privatePCA} and then feed the outputs to the neural network which is trained using local DPSGD algorithm described in \cite{dwork2014algorithmic}. Therefore, in this paper, we only consider comparisons with the local DPSGD algorithm for the neural network instead of differentially private PCA algorithm.

Consider MNIST dataset which has $N=60000$ examples, in local DPSGD \cite{dwork2014algorithmic}, the authors used the following settings for training process: the number of epochs E = 16, batch size B = 600, $(\epsilon,\delta)=(0.5,10^{-5})$, clipping norm C = 4, the noise for neural network and PCA projections are $(\sigma,\sigma_p) = (8,16)$ respectively, the number of iteration $K = \frac{E*N}{B} = \frac{16*60000}{600} = 1600$. However, according to \cite{dwork2014algorithmic}'s theorem 1, the smallest noise they can use are: $(\sigma,\sigma_p) = (\Omega(\frac{B}{N}*\sqrt{K*\log(\frac{1}{\delta})}/\epsilon),\sqrt{2*\log(\frac{1.25}{\delta})}/\epsilon) = (\Omega(\frac{600}{60000}*\sqrt{1600*\log(\frac{1}{10^{-5}})}/0.5),\sqrt{2*\log(\frac{1.25}{10^{-5}})}/0.5) \approx (\Omega(2.71),9.69)$. In our settings, with $N=60000,E=16,s = 600, \delta = 10^{-5}$, we can achieve $\epsilon \approx 0.61$ and $\sigma \approx 6.13$ which is smaller than the computed noise above. Another example for the similar privacy budget $(\epsilon,\delta) = (0.49,10^{-5})$, $N=60000,E=12,s = 600$, we only need $\sigma \approx 6.86$ to satisfy $(\epsilon,\delta)-DP$, this is also smaller than $\sigma = 8$ which is used in local DPSGD example in \cite{dwork2014algorithmic}. From above analysis, we can have the better accuracy for the MNIST dataset.
% Local DP-SGD papers

% Federated learning DP-SGD papers

% Secured Multiparty computation papers (optional)

% Compared with our paper...
